The Case for Learned In-Memory Joins

In-memory join is an essential operator in any database engine. It has been extensively investigated in the database literature. In this paper, we study whether exploiting the CDF-based learned models to boost the join performance is practical or not. To the best of our knowledge, we are the first to fill this gap. We investigate the usage of CDF-based partitioning and learned indexes (e.g., Recursive Model Indexes (RMI) and RadixSpline) in the three join categories; indexed nested loop join (INLJ), sort-based joins (SJ) and hash-based joins (HJ). Our study shows that there is a room to improve the performance of INLJ and SJ categories through our proposed optimized learned variants. Our experimental analysis showed that these proposed learned variants of INLJ and SJ consistently outperform the state-of-the-art techniques.

==> acknowledgement.tex <==
\begin{acks}
\label{sec:acknowledgment}

 %This work was supported by the [...] Research Fund of [...] (Number [...]). Additional funding was provided by [...] and [...]. We also thank [...] for contributing [...].

TO BE DONE

\end{acks}


==> introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}

In-memory join is an essential operator in any database engine. It has been extensively investigated in the database literature (e.g.,~\cite{HYF+08, HL06, AKN12, BAT+13, TAB+13, BLP11, LLA+15, BGN21}). Basically, in-memory join algorithms can be categorized into three main categories:~nested loop joins (e.g.,~\cite{HYF+08, HL06}), whether non-indexed or indexed, sort-based joins (e.g.,~\cite{AKN12, BAT+13}), and hash-based joins (e.g.,~\cite{TAB+13, BLP11, LLA+15, BGN21}). Many recent studies (e.g.,~\cite{BAT+13, SCD16}) have shown that the design, as well as the implementation details, have a substantial impact on the join performance, specially on the modern hardware.

Meanwhile, there has been growing interest in exploiting machine learning techniques to speed up the core database functionality and automate its design decisions. The key idea consists of augmenting, and sometimes even replacing, classic data structures and database operations, with machine learning models, which are better in exploiting trends in the input data and instance-optimizing the performance. This has led to recent advances in indexing~\cite{KBC+18, KMR+20, FV20}, query optimization~\cite{MNM+19, MNM+21}, cardinality estimation~\cite{KKR+19}, data partitioning~\cite{YCW+20}, and sorting~\cite{KVC+20}. Along this line of work, the authors of~\cite{KBC+18} suggested the idea of using {\cdf}-based learned models to improve the performance of join algorithms. However, this idea was never fully investigated.


In this paper, we study whether exploiting the {\cdf}-based learned models to boost the performance of in-memory joins is practical or not. In particular, we investigate how to efficiently use {\cdf}-based partitioning and learned indexes (e.g., Recursive Model Index ({\rmi})~\cite{KBC+18}) in the different phases of three join categories; indexed nested loop join ({\inlj}), sort-based joins ({\sj}) and hash-based joins ({\hj}). Although the learned model ideas have been introduced in previous works, none of them has been studied in the context of join processing. Through our study, we observed that using off-shelf learned models "as-is" in replacing phases of different join algorithms is sub-optimal. For example, the LearnedSort algorithm~\cite{KVC+20} can be used as a black-box replacement for the sorting algorithms used in the state-of-the-art {\sj} techniques, such as {\mpsm}~\cite{AKN12} and {\mway}~\cite{TAB+13}. However, this leads to repeating unnecessary work, and hence increases the overall execution time. Another example is replacing the hash functions used in hash-based {\inlj} with {\rmi} models. Unfortunately, this also leads to a poor performance (i.e., high overall latency) as computing a hash function is significantly faster than calculating a prediction using {\rmi}. Therefore, we argue that efficiently leveraging the learned models with in-memory joins is a challenge by itself, that needs to be addressed. In addition, succeeding to have efficient learned joins will help us to realize our vision of building an instance-optimized DBMS, like SageDB~\cite{KAB+19}.




We started with the {\inlj} category, where we first studied the most straightforward idea of directly using one input relation $R$ to build an {\rmi}, and then use the other input relation $S$ to probe this built {\rmi} for join matches. However, our results showed that this idea is not practical in many cases due to the significant overhead needed to correct the {\rmi} mispredictions. Therefore, we introduced two efficient variants of learned {\inlj} that overcome this issue. The first variant, namely Gapped {\rmi} {\inlj}, employs an efficient read-only {\rmi} that is built using the concept of \textit{model-based insertion} introduced in~\cite{DMY+20}. To further improve the performance of this variant, we introduced a new approach to buffer the probe (i.e., look up) operations over the {\rmi}, namely Requests Buffer, to reduce the cache misses, and hence improves the join throughput. We also provided a cache complexity analysis for this buffering technique, and proved its matching to the caching analytical bounds in~\cite{HL06}. The second variant, namely learned-based hash {\inlj}, employs {\rs} to build a hash index that is useful in some scenarios.

In {\sj} category, we proposed a new sort-based join, namely {\lsj}, that exploits a {\cdf}-based model to improve the different {\sj} phases (e.g., sort and join) by just scaling up its prediction degree. {\lsj} has the following two merits. First, it combines {\cdf}-based partitioning with AVX sort to provide a new efficient sorting phase. We also provided a complexity analysis for this new sorting phase. Second, it employs the {\cdf}-based model to reduce the amount of redundant join checks in the merge-join phase. In {\hj} category, we tried using the learned models in the different building and probing operations, however, we concluded that typical hash joins are always better.

In addition to the proposed learned join algorithms, we touch on the join query planning problem and introduce a simple \textit{joins optimizer} that selects which join algorithm to use a priori, whether learned or non-learned. The proposed optimizer is based on a simple reinforcement learning technique, referred to as the contextual multi-armed bandit~\cite{LPP10}, and automatically learns the join algorithm selection based on simple join features that are extracted from the query itself and its input data.


Our experimental evaluation shows that the proposed learned joins for {\inlj} and {\sj} provide the best performance against the state-of-the-art competitors in each category with different real ({\sosd}~\cite{MKR+20}) and synthetic datasets. For example, our Gapped {\rmi} {\inlj} can be 2.7X faster than hash-based {\inlj} in many scenarios and with different datasets. In addition, the proposed {\lsj} can be 2X faster than Multi-way sort-merge join~\cite{BAT+13}, which is the best sort-based join baseline in the literature.

%\footnote{anonymous.4open.science/r/learned-joins-C41D}

%To the best of our knowledge, we are the first to fill this gap. 






==> joins_optimizer.tex <==
\section{Bandit-based Joins Optimizer}
\label{sec:joins_optimizer}

\begin{figure}
    \begin{center}
     \includegraphics[width=3.2in]{figures/joins_optimizer.eps}
     \end{center}
     \caption{Overview of the Bandit-based Joins Optimizer.}
     \label{fig:joins_optimizer}
\end{figure}

Deciding which join algorithm to use a priori, whether learned or non-learned, is a challenging query planning problem~\cite{MNM+21}. However, to make full use of our proposed learned joins, we introduce a simple joins optimizer that automatically learns which join algorithm to use with each join query, based on simple join features extracted from the query itself and its input data. Although such optimizer is not comprehensive and not considering other operators in the query plan (e.g., select or aggregate), it is still useful to provide some basic guidance on the usage patterns of each join algorithm (Check Section~\ref{sec:evaluation} for learned lessons from this optimizer). 

We propose to use a simple reinforcement learning technique, referred to as the contextual multi-armed bandit~\cite{LPP10}, to build our joins optimizer, namely \textit{Bandit-based Joins Optimizer}. Figure~\ref{fig:joins_optimizer} shows an overview of its components. Whenever a join query arrives for execution, the \textit{Join Featureizer} extracts a set of simple features describing the join operation and its input (i.e., the context). Examples of these features include the input size, data type, distribution type if known, whether it is indexed or not, and the type of used index if exists. Then the extracted features are fed to the \textit{Join Selection Model}, which is typically a neural network, to select a join algorithm (i.e., the action) from a finite set (referred to as bandit arms). After running the join algorithm and receiving the query latency (i.e., the reward), the \textit{Collector} records a tuple consisting of the extracted features, join selection and the received latency as an experience for retraining the \textit{Join Selection Model} in the future. The goal of this model is to minimize the join query latency over time. The model uses Thompson sampling~\cite{CL11} to balance between \textit{exploring} the relationship between contexts, actions and rewards, and \textit{exploiting} the knowledge that is already gained. The initial model accuracy can be boosted in the beginning by using a training workload, if available.




==> learned_indexed_nested_loop_join_v1.tex <==
\section{Learned Indexed Nested Loop Join}
\label{sec:linlj}

In this section, we explore using the learned index idea in indexed nested loop joins ({\inlj}). One straightforward approach is to index one input relation, say $R$, with an {\rmi} and then use the other relation, say $S$, to probe the built {\rmi} and check for the join matches. This is an appealing idea because {\rmi}~\cite{KBC+18} typically encodes the built index as few linear model parameters (i.e., small index representation), and in turn improves the {\inlj} cache behavior. However, our experiments showed that using typical {\rmi}s only is not the best option in all cases. This is mainly due to the significant overhead of the "last-mile" search (i.e., correcting the {\rmi} mispredictions using binary search) when having challenging datasets. Therefore, we first propose a new variation of {\rmi} (Section~\ref{sec:linlj_gapped_rmi}) that substantially improves the "last-mile" search performance for general lookup queries (e.g., filtering), yet, with higher space requirements (i.e., less cache-friendly). Then, we provide a customized variation of this index (Section~\ref{sec:linlj_optimized_buffer}) for {\inlj} that exploits a cache-optimized buffering technique to increase the caching benefits while keeping the improved search performance during the {\inlj} processing. 

\subsection{Gapped {\rmi} ({\grmi})}
\label{sec:linlj_gapped_rmi}

\begin{figure}
    \begin{center}
    \includegraphics[width=3.2in]{figures/grmi.eps}
    \end{center}
    \caption{Example of 2-levels Gapped {\rmi} ({\grmi})}
    \label{fig:linlj_grmi}
\end{figure}


The performance of any {\inlj} algorithm mainly depends on the used index. However, when using {\rmi} in {\inlj} over challenging inputs, the join throughput deteriorates as the input data is difficult to learn and the accuracy of built {\rmi} becomes poor. In this case, the {\rmi} predicts a location which is far away from the true one, and hence the overhead of searching between the error bounds becomes significant. This is because when an {\rmi} is built for an input relation, it never changes the positions of the tuples in this relation. 
A key insight from a recent updatable learned index~\cite{DMY+20}, namely {\alex}, shows that when tuples are inserted using a learned model, the search over these tuples later, using the same model, will be improved significantly. 
Basically, \textit{model-based} insertion places a key at the position where the model predicts that the key should be. As a result, \textit{model-based} insertion reduces the model misprediction errors. 
This inspires us to propose a new read-only {\rmi}-based index, namely Gapped {\rmi} ({\grmi}), that substantially improves the lookup performance over typical {\rmi}, specially for datasets with challenging distributions.   
 
\noindent\textbf{{\grmi} Structure.} The proposed {\grmi} consists of a \textit{typical {\rmi}} and \textit{two gapped arrays}, one for keys and one for payloads. We assume both keys and payloads have fixed sizes. Any payload could be an actual record or a pointer to a variable-sized record, stored somewhere else. The gapped arrays are filled by model-based inserts of the input tuples (described later). The extra space used for the gaps is distributed among the elements of the array, to ensure that tuples are located closely to the predicted position when possible. The number of allocated gaps per input key is a user-defined parameter that can be tuned. For efficient lookup, the gapped arrays are associated with a bitmap to indicate whether each location in the array is filled or is still a gap. Figure~\ref{fig:linlj_grmi} depicts an example of a 2-levels {\grmi}, where we show only the gapped array for keys (white cells are gaps (i.e., empty)).

{\grmi} has two main differences from {\alex}. First, {\grmi} is a \textit{read-only} data structure which is built once in the beginning and then used for lookup operations only. In contrast, {\alex} is more dynamic and can support updates, insertions and deletes. Second, {\alex} is a B-tree-like data structure which has internal nodes containing pointers and storing intermediate gapped arrays. Unlike {\alex}, {\grmi} just has only two \textit{continuous} gapped arrays, for keys and payloads, to perform the "last-mile" search operations in an efficient manner. Note that {\grmi} employs a typical {\rmi} for predicting the key's location, without any traversal for internal nodes as in {\alex}. Therefore, the {\grmi} lookup is extremely efficient compared to {\alex} as shown in our experiments (Section~\ref{sec:evaluation}).  

\noindent\textbf{{\grmi} Building.} Building a {\grmi} has two straightforward steps. First, a typical {\rmi} is constructed for the input keys. Then, the built {\rmi} is used to model-based insert all tuples from scratch in the gapped arrays. \textit{Note that, in {\inlj}, the index is assumed to be existing beforehand}. This is a typical case in any DBMS where indexes (e.g., hash index, B-tree) are general-purpose and built once to serve many queries (e.g., select, join).  \textit{Therefore, the {\grmi} building overhead has no effect on the {\inlj} performance}. 

\noindent\textbf{{\grmi} Lookup.} Given a key, the {\rmi} is used to predict the location of that key in the gapped array of keys, then, if needed, an \textit{exponential search} is applied till the actual location is found. If a key is found, we return the corresponding payload at the same location in the payloads array, otherwise return null. We use the exponential search to find the key in the neighborhood because, in {\grmi}, the key is likely to be very close to the predicted {\rmi} location, and in this case, the exponential search can find this key with less number of comparison checks compared to both sequential and binary searches. Figure~\ref{fig:linlj_grmi} presents a lookup example, where red arrows show the lookup flow. In this example, the {\rmi} prediction is corrected by two exponential search steps only.


%\subsection{Request Buffers Optimization}
\subsection{Buffered {\grmi} {\inlj}}
\label{sec:linlj_optimized_buffer}

\begin{figure}
    \begin{center}
    \includegraphics[width=3.2in]{figures/rmi_requests_buffer.eps}
    \end{center}
    \caption{{\rmi} Structure with Request Buffers (buffer for each model).}
    \label{fig:linlj_buffer}
\end{figure}

Although leveraging the model-based insertion and exponential search ideas in {\grmi} reduces the number of comparisons and their corresponding cache misses in the "last-mile" search, directly using {\grmi} in {\inlj} is sub-optimal as it introduces another kind of cache misses when iteratively looking up for different keys. Since  keys are stored in quite large gapped arrays in {\grmi}, the probability of finding different keys within the same cacheline is low. To address this issue, we propose to buffer (i.e., temporarily store) the requests for query keys that will be probably accessed from the same part in the \textit{gapped array} (i.e., keys that predict the same models across the {\rmi} levels), and then answer them as a batch. This significantly improves the temporal locality of the index, reduces cache misses, and in turn increases the join throughput.
In this section, we show how we adapt an efficient variation of \textit{hierarchical} buffering techniques~\cite{ZR03, HL06} to improve the throughput of {\inlj} using {\grmi}. We refer to this variation as \textit{Buffered {\grmi}} ({\bgrmi}).

\noindent\textbf{Key Idea.} We view the {\rmi} as a tree with multiple sub-trees rooted at the child models, and the root of each sub-tree is associated with a fixed-size buffer. We refer to this buffer as \textit{request buffer}, where it temporarily stores all keys that will be predicted using the corresponding child model. Figure~\ref{fig:linlj_buffer} shows the first 3 levels of an {\rmi}, where the root of each sub-tree (i.e., child model) has a request buffer. The dotted lines represent a sub-tree. For example, the "Root" model has two sub-trees rooted at its child models "$M 1.1$" and "$M 1.2$". Recursively, the "$M 1.1$" model has two sub-trees rooted at "$M 2.1$" and "$M 2.2$". The buffer at "$M 1.1$" is used to store the keys that already predicted "$M 1.1$" at the current level, and will predict models from its sub-tree in the future.

The request buffers for all sub-trees of the indexed relation, say~$R$, are created before the {\inlj} begins. During the {\inlj} operation, the query keys from the non-indexed relation, say $S$, are distributed to the buffers based on the {\rmi} predictions, until a buffer becomes full. When a buffer is full, we flush it by distributing the buffered query keys to its child buffers recursively. When a query key reaches the leaf-level, the final {\rmi} prediction is performed. When no more query keys are issued, the whole request buffers are flushed in the depth-first order similar to~\cite{HL06}. 
However, defining a request buffer for "every" sub-tree in {\rmi} is unnecessary and will result in cache misses when accessing the buffers themselves, specially in case of having large {\rmi} (i.e., large number of request buffers). \textit{Therefore, as an optimization, we recursively apply the request buffers on the {\rmi} index, until a sub-tree $t$ and its buffers (excluding the buffer of this sub-tree's root) totally fit into the cache and then stop. }

%However, determining the sizes of these request buffers is challenging for two main reasons. First, the size of each {\rmi} node's buffer depends on the node's level and the {\rmi}'s fan-out (i.e., number of child models at level $i+1$ for a parent model at level $i$). Second, these buffers should fit in the cache, otherwise their benefit will be diminished by cache misses coming from accessing the buffers themselves.

During the rest of this section, we discuss how the proposed buffering and its optimization satisfy the analytical bound of the \textit{cache complexity} in hierarchical indexes (e.g., trees or {\rmi})~\cite{HL06}. The cache complexity is defined by the asymptotic number of block transfers between the cache and the memory incurred by a query key. First, we derive an upper bound on the total size of request buffers needed for an {\rmi}. Then, we use this upper bound in deriving the cache complexity.

\noindent\textbf{Total Buffers' Size Upper Bound.} Here, we present a worst-case bound on the total size of request buffers needed by an {\rmi}. Note that our goal is to maximize the {\inlj} performance with {\rmi} and its variant {\grmi}, not to minimize the buffer sizes. Therefore, this analysis is useful for gaining intuition about request buffer sizes, but does not reflect worst-case guarantees in practice.

Assume an {\rmi} rooted at the model $r$. Let $n$ be the total number of models (all intermediate and leaf models) in this {\rmi}, $m$ is its fan-out (i.e., number of children per model). Also, assume that $w$ is the fixed-size, in bytes, of a single model in this {\rmi}. We define $S(n)$ to be  the total size of request buffers associated with the $n$ models of this {\rmi}, \textit{without the buffer size needed at the root $r$}. We set the buffer size needed at the root $r$ to be $wn + S(n)$ (i.e., equals to the total size of all $n$ models in this {\rmi} ($wn$) and the buffers for its non-root models $S(n)$). This is intuitive because if the {\rmi} nodes and all their buffers (excluding the buffer for the root node) fit into the cache, they can be reused before eviction from the cache. \\

\begin{proposition}
\textit{Given an {\rmi} with number of intermediate and leaf models $n$ (without the root), child fan-out $m$ and model size $w$, the total size, in bytes, needed for the request buffers $S(n)$ is $O(n \log_m n)$.}
\label{prop:request_buffer_size}
\end{proposition}

\begin{proof}
As previously mentioned, an {\rmi} with fan-out of $m$ can be viewed as a tree that starts from the root model $r$. Such tree consists of $m$ sub-trees; each sub-tree starts from one of the $m$ child models of $r$. Since the whole {\rmi} tree contains $n$ models, then each of these sub-trees $t$ roughly contains $\frac{n}{m}$ nodes. From our definitions, the total size of buffers needed for each sub-tree $t$, without the buffer needed for the root of $t$, is $S({\frac{n}{m}})$. In addition, the size of buffer at the root itself is $w\frac{n}{m} + S(\frac{n}{m})$. Hence, we can redefine $S(n)$ in terms of $S(\frac{n}{m})$ to be as follows:  


\begin{equation}
S(n) = m (w\frac{n}{m} + 2S(\frac{n}{m})) = wn + 2m S(\frac{n}{m}) 
\label{eq:buffer_size}
\end{equation}

By solving this equation recursively, we end up with $S(n) = wn (1 + 2 + \ldots + \log_m n) + (2m)^{\log_m n}$, where $(1 + 2 + \ldots + \log_m n)$ is a geometric series. After eliminating lower-order terms of this series and assuming $n \gg m$, $S(n)$ becomes $O(n \log_m n)$ ($w$ is omitted as it is constant). \\

\end{proof}

Equation~\ref{eq:buffer_size} is used to automatically estimate the buffer size at each model (sub-tree root) in {\rmi}, in a recursive manner, starting from the leaf level and up to the root. Note that the assumption of $n \gg m$ is valid as, in practice, the {\rmi} optimizer~\cite{MZK20} typically models a large input relation with complex distribution using {\rmi} of 2 to 3 levels (excluding the root), and a fan-out $m$ of 1000. In the case of 2 levels, for example, the $\frac{n}{m}$ ratio becomes 1000, which is relatively large. 

\noindent\textbf{Request Buffers Cache Complexity.} Assume $B$ is the cache line size in bytes, and $C$ is the cache capacity in bytes. According to~\cite{HL06}, the amortized cache complexity of one probe using the buffering scheme of a hierarchical index $X$ (e.g., trees or {\rmi}) should be less than or equal to $O(\frac{1}{B} \log_C n)$, where $n$ is the number of index nodes ({\rmi} models in our case). Otherwise, this buffering scheme is considered inefficient. Here, we show that our request buffers match the analytical bound of probing cache complexity, and hence proved to be efficient. \\

\begin{proposition}
\textit{The amortized cache complexity of one probe using our request buffers is $O(\frac{1}{B} \log_C n)$, where $n$ is the number of {\rmi} models, and hence matches the analytical bound from~\cite{HL06}.}
\label{prop:request_buffer_cache_complexity}
\end{proposition}

\begin{proof}
As mentioned before, we recursively apply the request buffers on the {\rmi} index, until a sub-tree $t$ and its buffers (excluding the buffer of this sub-tree's root) totally fit into the cache. Assume the number of models in this sub-tree $t$ is $k$. Then, using Proposition~\ref{prop:request_buffer_size}, the total size of the sub-tree $t$ and its buffers, excluding the buffer at $t$'s root, can be represented using this inequality $w(k \log_m k) < C$. By taking $\log_m$ for both sides, $(\log_m k + \log_m \log_m k) < \log_m \frac{C}{w}$. After eliminating lower-order terms, $\log_m k < \log_m \frac{C}{w}$.


Assume the size of probe key in bytes is $q$. Since we are using fixed-size buffers, the amortized cost of each probe on a sub-tree that fits in the cache is $O(\frac{1}{B})$, because the cost of loading sub-tree into the cache is amortized among $\frac{w(k \log_m k)}{q}$ probes. In addition, the number of sub-trees fitting in the cache that each probe should go through is $O(\frac{\log_m n}{\log_m k}) = O(\frac{\log_m n}{\log_m C}) = O(\log_C n)$. As a result, the amortized cost of each probe on the {\rmi} index is $O(\frac{1}{B} \log_C n)$, and meets the analytical bound in~\cite{HL06}. \\

\end{proof}


\subsection{Learned-based Hash {\inlj}}
\label{sec:linlj_rmi_hash}

Instead of directly using a learned index (e.g., {\rmi} or {\rs}~\cite{KMR+20}) in {\inlj}, we can employ a variant of a hash index that uses the learned index to build and probe its hash table (i.e., the learned index is used as a hash function)~\cite{SVH+21}. Basically, if the input keys are generated from a certain distribution, then the {\cdf} of this distribution maps the data uniformly in the range $[0, 1]$, and the {\cdf} will behave as an order-preserving hash function in a hash table. In some cases, the {\cdf}-based models in the learned index can over-fit to the original data distribution, and hence results in less number of collisions compared to traditional hashing, which would still have around 36.7\% regardless of the data distribution (based on the birthday paradox). For example, if the data is generated in an incremental time series fashion, or from sequential data with holes (e.g., auto generated IDs with some deletions), the predictability of the gaps between the generated elements determines the amount of collisions, and can be captured accurately using learned models. Note that we build the learned index using the entire input relation, and hence its accuracy becomes high. Our experimental results (Section~\ref{sec:evaluation}) show the effectiveness of the learned-based hash variant in some real and synthetic datasets.



%% We might need to talk about RadixSpline here... or in the worst case in the experiments....

==> optimizations.tex <==
\section{Performance Optimizations}
\label{sec:optimizations}

TO BE DONE

%\subsection{{\imv}-based Primitives}
%\label{sec:imv_primitives}

%\begin{itemize}
%    \item Providing details for IMV CDF-based Scattering and Gathering primitives
%    \item Providing algorithms for each primitive
%\end{itemize}

%\subsection{Revisiting Learned Joins}
%\label{sec:revisiting_learned_joins}

%\begin{itemize}
%    \item Discussing how these primitives are used to improve the previously discussed learned joins
%\end{itemize}
